The orbifold Hochschild product for Fermat hypersurface

Let $G$ be an abelian group acting on a smooth algebraic variety $X$. We investigate the product structure and the bigrading on the cohomology of polyvector fields on the orbifold $[X/G]$, as introduced by C\u{a}ld\u{a}raru and Huang. In this paper we provide many new examples given by quotients of Fermat hypersurfaces, where the product is shown to be associative. This is expected due to the conjectural isomorphism at the level of algebras between the cohomology of polyvector fields and Hochschild cohomology of orbifolds. We prove this conjecture for Calabi-Yau Fermat hypersurface orbifold. We also show that for Calabi-Yau orbifolds, the multiplicative bigrading on the cohomology of polyvector fields agrees with what is expected in homological mirror symmetry.

==> definition.tex <==
\section{Definition of the product on orbifold polyvector fields}

In this section we define the product on orbifold polyvector fields.
The technical results used in the definition are introduced
in this section, but will be proved in Section 4.

As we have explained previously, the Hochschild cohomology and the
polyvector fields cohomology of a space $X$ can be viewed as the
distributions on the derived loop space (a derived Lie group) and on
its Lie algebra, respectively.  The product structures on these come
from the convolution of distributions.  We begin by recalling the
definition of the convolution product of distributions on (classical)
Lie groups and Lie algebras.

\paragraph{\bf Distributions on Lie groups and Lie algebras.}  Let $G$
be a Lie group with Lie algebra $\g$.  The convolution product of
distributions $\bD(G)$ on $G$ is defined as follows
$$ \xymatrix{ \bD(G)\otimes\bD(G)\ar[r] &
  \bD(G\times G)\ar[r]^{m_*} &\bD(G), }$$ where $m$ is the
multiplication map $G\times G\rightarrow G$, and $m_*$ is the induced
map on distributions.  The Lie algebra $\g$ of $G$ is a vector space.
It is considered as an abelian group under the addition operation of
vectors.  One can define the convolution product for $\bD(\g)$
similarly.

In the derived setting, the convolution product on orbifold Hochschild
cohomology is known as the composition of morphisms in the derived
category.  We hope to define the convolution product on the polyvector
fields.  Therefore, it is important to know how to recover the
convolution product on $\bD(\g)$ with the knowledge of the group $G$
only.  The following is how we do this.

First there is a multiplication map $m:G\times G\rightarrow G$.
Taking derivative of this map, we get the induced map on tangent
spaces $\bL_m: \bL_{G\times G}\rightarrow \bL_G$, where $\bL_G=\g$
is the tangent space of $G$ at origin.  We use the same notation $\bL$
as the notation for the linearization of derived schemes in the
derived setting.

There is a natural isomorphism $\bL_{G\times
G}\cong\bL_G\times\bL_G$.  Under this natural identification, the map
$\bL_m:\bL_G\times\bL_G\rightarrow\bL_G$ is nothing but the addition
law on the vector space $\bL_G$.  We can recover the convolution
product of $\bD(\bL_G)$ now $$\xymatrix{
\bD(\bL_G)\otimes\bD(\bL_G)\ar[r] &
\bD(\bL_G\times\bL_G)\ar[r]^{\cong} &\bD(\bL_{G\times
G})\ar[r]^{{\bL_m}_*} & \bD(\bL_G). } $$

\paragraph{\bf A non-trivial isomorphism in the derived setting.} We
can try to do exactly the same thing in the derived setting.  However,
there is a technical issue.  The natural isomorphism $\bL_{G\times
G}\cong\bL_G\times\bL_G$ is not at all obvious for the derived loop
space.  The analogous statement would be
\[ \bL_{L\sX\times_{\sX}^R  L\sX}\cong\bL_{L\sX}\times^R_{\sX}\bL_{L\sX} \]
for the derived loop space of an orbifold $\sX$.  The left hand side
is obviously linear: it is a total space of a vector bundle over the
inertia stack $I\sX$.  On the other hand, it is not at all obvious
that the right hand side can be linearized.

The following two propositions will be proved in the next sections.

\begin{Proposition}
  \label{Prop formality}
  Let $\sX=[X/G]$ be a global quotient orbifold of a finite group $G$
  acting on a smooth algebraic variety.  If we further assume $G$ is
  abelian, then there is an isomorphism
  \[ \bL_{(L\sX\times_{\sX}^R L\sX)}\cong\bL_{L\sX}\times^R_{\sX}\bL_{L\sX}. \]
\end{Proposition}

The derived loop space $L\sX$ decomposes naturally into connected
components, so we can restate the above proposition on components.

\begin{Proposition}
  \label{Prop formality'}
  In the same setting as Proposition \ref{Prop formality}, there is an
  isomorphism
  \[
    \bL_{\widetilde{X^g}\times^R_X\widetilde{X^h}} \cong
    \bL_{\widetilde{X^g}} \times^R_X\bL_{\widetilde{X^h}} \] 
  for any $g,h\in G$.
\end{Proposition}
\medskip

\paragraph{\bf The definition of the convolution product in the
  derived setting.}
The multiplication map for Lie groups plays an important role in the
case of Lie groups and Lie algebras.  We need to know what the
multiplication map is for the derived loop space
$L\sX=\sX\times^R_{\sX\times\sX}\sX$ of $\sX$.  It is the projection
map $p_1\times p_3$ onto the first and the third factors
\[ \xymatrix{
    L\sX\times_{\sX}L\sX\ar[r]^{m}\ar[d]^{=} & L\sX\ar[d]^{=}.\\
    \sX\times^R_{\sX\times\sX}\sX\times^R_{\sX\times\sX}\sX\ar[r]^{~~~~~~p_1\times
      p_3} & \sX\times^R_{\sX\times\sX}\sX. } \]

We need three lemmas for derived groups which are generalizations of
well-known results from classical Lie group theory.

\begin{Lemma}
  \label{lem induced map on linearizations}
  A map $f: X\longrightarrow Y$ between derived schemes induces a map on
  linearlizations $\bL_f:\bL_{X}\longrightarrow\bL_Y$.
\end{Lemma}

\begin{proof} We have a commutative diagram $$ \xymatrix{ X^0
\ar[d]^{i} \ar[r]^{g} & Y^0 \ar[d]^{j} \\ X \ar[r]^{f} & Y, } $$

where $X^0$ and $Y^0$ are the classical schemes of $X$ and $Y$
respectively.  Then there is a commutative diagram of derived tangent
complexes $$ \xymatrix{ T_{X^0} \ar[d] \ar[r] & g^*T_{Y^0} \ar[d] \\
i^*{T}_{X} \ar[r] & i^*f^*{T}_{Y}=g^*j^*{T}_{Y}.  } $$

Passing to the quotient, we get an induced
map $$N_{X^0/X}=i^*{T}_{X}/T_{X^0}\rightarrow
g^*(j^*{T}_{Y})/g^*T_{Y^0}=g^*(j^*{T}_{Y}/T_{Y^0})=g^*N_{Y^0/Y}.$$

The map above is equivalent to a map $\bN_{X^0/X}\rightarrow
\bN_{Y^0/Y}\times_{Y^0}X^{0}$ in terms of total spaces. \end{proof}

Applying the above lemma to the multiplication map of derived loop
space yields an induced map
$\bL_m:\bL_{L\sX\times^R_{\sX}L\sX}\rightarrow\bL_{L\sX}.$

\begin{Lemma}
  \label{lem push-forward of dist}
  Suppose there is a commutative diagram
  $$\xymatrix{ X \ar[rr]^f\ar[dr]_i & & Y\ar[dl]^j \\ & S & }$$ of
  (derived) schemes.  Then there is a pushforward map for relative
  distributions, i.e., there is a natural induced map
  $f_*:\bD(X/S)\rightarrow\bD(Y/S).$
\end{Lemma}

\begin{proof}
  We have $\bD(X/S)=\Hom(i_*\cO_X,\cO_S)$.  Applying $j_*$ to the map
  $\cO_Y\rightarrow f_*\cO_X$, we get a map
  $j_*\cO_Y\rightarrow j_*f_*\cO_X=i_*\cO_X$.  Composing it with
  $i_*\cO_X\rightarrow \cO_S$, we get the desired pushforward map.
\end{proof}

\begin{Lemma}
  \label{lem tensor prod of dist}
  Suppose there is a commutative diagram
  $$ \xymatrix{ W=X\times^R_SY\ar[r]\ar[d]\ar[dr]^\pi & Y\ar[d]_j \\
    X\ar[r]^i & S} $$ of (derived) schemes.  Then there is a natural map
  $\bD(X/S)\otimes\bD(Y/S)\rightarrow\bD(W/S)$.
\end{Lemma}

\begin{Proof}
  We have
  \begin{align*}
    \Hom(i_*\cO_X,\cO_S)\otimes\Hom(j_*\cO_Y,\cO_S) & \ra
    \Hom(i_*\cO_X\otimes_{\cO_S}   j_*\cO_Y,\cO_S) \\
                                                    &
                                                      =\Hom(\pi_*\cO_W,\cO_S). 
  \end{align*}
  \vspace*{-4em}
  
\end{Proof}

With the three lemmas above we are able to define our desired
product.

\begin{Definition}
\label{def product}
Under the assumptions in Proposition~\ref{Prop formality} we define
the following binary operation on $\bD(\bL_{L\sX}/\sX)$, which is our
proposed definition for a product on orbifold polyvector fields:.
\begin{align*}
  \bD(\bL_{L\sX}/\sX)\otimes\bD(\bL_{L\sX}/\sX) & \lra
      \bD(\bL_{L\sX}\times^R_{\sX}\bL_{L\sX}/\sX) \stackrel{\sim}{\lra}
      \bD(\bL_{(L\sX\times_{\sX} L\sX)}/\sX) \\
      & \stackrel{\bL_{m_*}}{\lra}\bD(\bL_{\sX}/\sX), 
\end{align*}
where the first arrow is due to Lemma \ref{lem tensor prod of dist},
the second arrow is the non-trivial isomorphism in Proposition
\ref{Prop formality}, and the last map is due to Lemmas \ref{lem
  induced map on linearizations} and \ref{lem push-forward of dist}.
\end{Definition}
\medskip

Looking at each connected component of $L\sX$ individually, the
definition gives a map for every $g, h\in G$
\[
  \bD(\bL_\tXg/X)\otimes\bD(\bL_\tXh/ X) \ra
    \bD(\bL_\tXg\times^R_{X}\bL_\tXh/
    X)\stackrel{\sim}{\lra} \bD(\bL_{(\tXg\times_{X}
      \tXh)}/ X)\stackrel{\bL_{m_*}}{\lra}
    \bD(\bL_{\tXgh}/ X). 
\]

